Exploiting Social Tie Structure for Cooperative Wireless Networking: A Social Group Utility Maximization Framework

In this paper, we develop a social group utility maximization (SGUM) framework for cooperative wireless networking that takes into account both social relationships and physical coupling among users. We show that this framework provides rich modeling flexibility and spans the continuum between non-cooperative game and network utility maximization (NUM) -- two traditionally disjoint paradigms for network optimization. Based on this framework, we study three important applications of SGUM, in database assisted spectrum access, power control, and random access control, respectively. For the case of database assisted spectrum access, we show that the SGUM game is a potential game and always admits a socially-aware Nash equilibrium (SNE). We develop a randomized distributed spectrum access algorithm that can asymptotically converge to the optimal SNE, derive upper bounds on the convergence time, and also quantify the trade-off between the performance and convergence time of the algorithm. We further show that the performance gap of SNE by the algorithm from the NUM solution decreases as the strength of social ties among users increases and the performance gap is zero when the strengths of social ties among users reach the maximum values. For the cases of power control and random access control, we show that there exists a unique SNE. Furthermore, as the strength of social ties increases from the minimum to the maximum, a player's SNE strategy migrates from the Nash equilibrium strategy in a standard non-cooperative game to the socially-optimal strategy in network utility maximization. Furthermore, we show that the SGUM framework can be generalized to take into account both positive and negative social ties among users and can be a useful tool for studying network security problems.

==> Framework.tex <==
\section{\label{sec:SGUF}Social Group Utility Maximization Framework}
Mathematically, we can model the database assisted  distributed spectrum access problem with social tie as a physical-social game formulation. Let $\mathcal{N}=\{1,2,...,N\}$ denote the set of white-space device users and $\mathcal{M}=\{1,2,...,M\}$ denote the set of white-space channels. By consulting the geo-location database, each device user $n$ can obtain the set of vacant channels $\mathcal{M}_{n}\in\mathcal{M}$ for data transmission. Each device user $n$ then chooses a feasible channel $a_{n}$ from the vacant channel set $\mathcal{M}_{n}$ for data transmission. Based on the channel selection profile of all device users $\boldsymbol{a}=(a_{1},...,a_{N})$, we introduce the \emph{individual utility function}   $U_{n}(\boldsymbol{a})$ to represent the payoff of of user $n$ due to the physical coupling of device users in data transmission. For example, $U_{n}(\boldsymbol{a})$ can be the achieved data rate or the satisfaction of quality of service (QoS) requirement of device user $n$ under the channel selection profile $\boldsymbol{a}$. For the social coupling, we introduce the social graph $\mathcal{G}^{S}$ to model the social tie among the device users. There is an social link between two device users if and only if they have social tie between each other, which can be kinship, friendship, or colleague relationship between two device users. Furthermore, we formalize
the strength of social tie between two device users $n$ and $m$ who have a social edge between them on the social graph as $w_{nm}\in[0,1]$,
with a higher value of $w_{nm}$ being a stronger social tie. Based on the social graph model, we further define the \emph{social group utility} of each device user $n$ as
\begin{equation}
S_{n}(\boldsymbol{a})=U_{n}(\boldsymbol{a})+\sum_{m\in\mathcal{N}_{n}^{s}}w_{nm}U_{m}(\boldsymbol{a}),\label{eq:SocialUtility}
\end{equation}
where $\mathcal{N}_{n}^{s}$ denotes the set of device users that have social tie with device $n$. The social group utility $S_{n}(\boldsymbol{a})$ of each device user consists two parts: his (her) individual utility
and the weighted sum of the individual utilities of other users having
social tie with him. The social group utility function captures the feature that each device
user is social aware and cares about the users having social tie with him.


The distributed spectrum access problem with social
tie is then given as follow. Given other device users' channel selections $a_{-n}$, each device user $n$
wants to choose a proper channel $a_{n}\in\mathcal{M}_{n}$ to maximize
his (her) social group utility, i.e.,
\[
\max_{a_{n}\in\mathcal{M}_{n}}S_{n}(a_{n},a_{-n}),\forall n\in\mathcal{N}.
\]
The distributed nature of the channel selection problem naturally
leads to a formulation based game theory, such that each device user
can self-organize into a stable channel selection (\emph{Nash equilibrium})
$\boldsymbol{a}^{*}=(a_{1}^{*},...,a_{N}^{*})$ wherein no user can
improve unilaterally, i.e.,
\[
a_{n}^{*}=\arg\max_{a_{n}\in\mathcal{M}_{n}}S_{n}(a_{n},a_{-n}),\forall n\in\mathcal{N}.
\]
We thus formulate the distributed spectrum access problem with social
tie as a \emph{physical-social game} formulation $\Gamma=(\mathcal{N},\{\mathcal{M}_{n}\}_{n\in\mathcal{M}_{n}},\{S_{n}\}_{n\in\mathcal{M}_{n}})$,
where the set of device users $\mathcal{N}$ is the set of players,
the set of vacant channels $\mathcal{M}_{n}$ is the set of strategies
for each user $n$, and the social group utility function
$S_{n}$ of each user $n$ is the payoff function of player $n$.



%\begin{figure}[tt]
%\begin{center}
%\includegraphics[scale=0.8]{ProblemSpectrum}
%\caption{\label{fig:Spectrum}Distributed spectrum access problem formulations with different users' social awareness levels}
%\end{center}
%\end{figure}

We would like to emphasize that, by using different social graphs, the proposed social-physical game formulation can provide rich flexibility for modeling the distributed spectrum access problem (see Figure \ref{fig:Spectrum} for an illustration). When the social graph consists of isolated nodes (i.e., all device users are selfish), the social-physical game degenerates to the non-cooperative game formulation for distributed spectrum access. When the social graph is fully meshed with edge weight $w_{nm}=1$ (i.e., each user is social aware and cares enough about other users), the social-physical game becomes the social welfare optimization problem, which aims to maximize the system-wide utility. The social-physical game formulation in this paper allows general social graphs and hence is feasible for modeling more general application scenarios. For example, we can consider the scenario that different device users belong to different authorities (e.g, network operators).  In this case, the users that belong to the same authority would like maximize their utilities collectively and meanwhile they will compete with other device users that are from other authorities. The social-physical game formulation can model such a scenario by defining the social graph in which the device users belonging to the same authority are connected with each other.
 
